On the Curses of Future and History in Future-dependent Value Functions for Off-policy Evaluation

We study off-policy evaluation (OPE) in partially observable environments with complex observations, with the goal of developing estimators whose guarantee avoids exponential dependence on the horizon. While such estimators exist for MDPs and POMDPs can be converted to history-based MDPs, their estimation errors depend on the state-density ratio for MDPs which becomes history ratios after conversion, an exponential object. Recently, Uehara et al. [2022a] proposed future-dependent value functions as a promising framework to address this issue, where the guarantee for memoryless policies depends on the density ratio over the latent state space. However, it also depends on the boundedness of the future-dependent value function and other related quantities, which we show could be exponential-in-length and thus erasing the advantage of the method. In this paper, we discover novel coverage assumptions tailored to the structure of POMDPs, such as outcome coverage and belief coverage, which enable polynomial bounds on the aforementioned quantities. As a side product, our analyses also lead to the discovery of new algorithms with complementary properties.

==> app/app_mis.tex <==
\section{New Algorithm} \label{sec:alg}
%The discovery of effective history weights and its boundedness also leads to a new algorithm analogous to MIS methods for MDPs \citep{uehara2019minimax}. 
Here we provide full details of the new MIS algorithm in Section~\ref{sec:mis_short}. 
The idea is that since \cref{lem:evaluation_error} tells us to minimize $\E_{\pie}[(\BES V)(s_h)]$, which equals $\E_{\pib}[w^\star(\tau_h) (\BEH V)(\tau_h)]$ from Def~\ref{def:his}, we can then use another function class $\Wcal \subset (\Hcal \to \RR)$ to model $w^\star$, and approximately solve the following:
\begin{align} \label{eq:MVL-alg}
\argmin_{V\in\Vcal} \max_{w\in\Wcal} \textstyle \sum_{h=1}^H |\E_{\pib}[w(\tau_h) (\BEH V)(\tau_h)]|,
\end{align}
which minimizes an upper bound of $\E_{\pib}[w^\star(\tau_h) (\BEH V)(\tau_h)]$ as long as $w^\star \in \Wcal \subset (\Hcal \to \RR)$. Since there is no square inside the expectation, there is no double-sampling issue and we thus do not need the $\Xi$ class and its Bellman-completeness assumption. % and replace it with the $\Wcal$ class that needs to realize $w^\star$ (or any other bounded solution to Def~\ref{def:his}). 
The $h$-th term of the loss can be estimated straightforwardly as
\begin{align} \label{eq:alg-estm}
|\E_{\Dcal} \left[w(\tau_h) \pa{\mu(o_h,a_h)\pa{r_h+ V(f_{h+1})} -V(f_h)}\right]|.\hspace*{-.1em}
\end{align}

We now provide the sample-complexity analysis of the algorithm, using a more general analysis that allows for approximation errors in $\Vcal$ and $\Wcal$. 

\begin{assumption}[Approximate realizablity]\label{asm:realize}
Assume
\begin{align*}
&\min_{V \in \Vcal} \max_{w \in \Wcal}\left|\sum_{h=1}^H \E_{\pi_b}\bra{w_h(\tau_h)\cdot (\BEH V)(\tau_h) }\right| \le \epsV, \\
&\inf_{w \in \lspan(\Wcal)} \max_{V \in \Vcal} \left|\sum_{h=1}^H \E_{\pi_b} \left[(w_h^\star(\tau_h) - w_h(\tau_h)) \cdot (\BEH V)(\tau_h)\right]\right| \qquad \le \epsW.
\end{align*}
\end{assumption}
%An interesting aspect of Assumption~\ref{asm:realize} is that, 
Instead of  measuring how $\Wcal$ and $\Vcal$ capture our specific constructions of  $\Vf$ and $w^\star$, the above approximation errors automatically allow all possible solutions by measuring the violation of the equations that define $\Vf$ and $w^\star$. 

We present the sample complexity bound of our algorithm as follows. Similar to Theorem~\ref{thm:finite_2}, we assume that $C_{\Vcal}:= \max_{V\in\Vcal} \|V\|_\infty$ and $C_{\Wcal} := \max_{h} \sup_{w\in\Wcal}  \|w\|_\infty$ are not much larger than the corresponding norms of $\Vf$ and $w^\star$, respectively. See the proof in Appendix~\ref{app:bound_weight}. % worst-case norms ($\|\cdot\|$ and $\|\cdot\|_{2, \db_h}$) close to the functions which these class are supposed to capture ($\Vf$ and $w^\star$). 
\begin{restatable}{theorem}{p1}
\label{thm:p1} \label{thm:bound_weight}
Let $\Vhat$ be the result of approximating Eq.\ref{eq:MVL-alg} with empirical estimation in Eq.\eqref{eq:alg-estm}. Assume that $C_{\Vcal} \le c \|\Vf\|_\infty$ for $\Vf$ in Eq.\eqref{eq:Vf-sol}, and $C_{\Wcal}  \le c \|w^\star\|_{\infty}$ for $w^\star$ in Eq.\eqref{eq:w-sol}. Under Assumptions~\ref{asm:belief_inf}, \ref{asm:outcome-inf}, and \ref{asm:realize},  w.p.~$\ge 1-\delta$, $\left|J(\pi_e) - \E_{\Dcal}[\Vhat(f_1)]\right| \le 
\epsV + \epsW + cH^2  \CHi (\CFi+1)\sqrt{\frac{C_{\mu} \log\frac{|\Vcal||\Wcal|}{\delta}}{n}}.$ 
\end{restatable}
%In addition to the approximation error, the bound aligns with the results in \cref{thm:finite_2}. This consistency demonstrates that our quantities in the coverage assumptions are general and not tailored to specific algorithms.

As a remark, there is also a way to leverage the tighter $L_2$ belief coverage, despite that it does not guarantee bounded $\|w^\star\|_\infty$ and only $\|w^\star\|_{2, \db_h}^2$. In particular, if all functions in $\Wcal$ have bounded $\|\cdot\|_{2, \db_h}^2$, the estimator in Eq.\eqref{eq:alg-estm} will have bounded 2nd moment on the data distribution. In this case, using Median-of-Means estimators \citep{lerasle2019lecture, chen2020short} instead of plain averages for Eq.\eqref{eq:alg-estm} will only pay for the 2nd moment and not the range.

==> app/app_response.tex <==
\section*{Response to ICML Meta-Review}

In NeurIPS 2020 and 2021, authors were asked to summarize how their papers have changed in light of reviews in previous rejections. Our work was reviewed for ICML 2024, and the meta-review made a number of inaccurate or technically incorrect claims about our work, where the Area Chair was likely confused by a long and convoluted discussion we had with one of the reviewers. We voluntarily included a response below to address these issues.

\subsection*{Polynomial vs.~Exponential}

\paragraph{Meta-review:} {\it ``authors' claim that `There were simply no polynomial sample complexity guarantees for OPE in POMDPs' \ldots there are existing works [with] $\sqrt{N}$ sample complexity where $N$ is the number of trajectories. \ldots I think the authors implicitly compares the results in terms of the coverage assumption.''}  

\paragraph{Response:} The meta-review missed the point. \textbf{The ``polynomial vs.~exponential'' discussion is never about rate in $N$, but dependence on horizon and other problem-dependent quantities}. This was made \textbf{clear and explicit} in the paper itself. We admit that that particular openreview post might not carry with it all the nuances, but we quickly clarified in follow-up posts. Also, \textbf{even the reviewer who raised the question understood the point} and had discussion with us on whether e.g., \citet{hu2023off}'s dependence on mixing time should be considered exponential. 

% We still stand by the point, but chose \textbf{not} to write like this in the actual paper (both the ICML submission and this manuscript), precisely because of all the nuances , and instead described our results in more concrete technical terms. 

\paragraph{Meta-review:} {\it ``this argument would benefit from a further refinement and detailed elaboration.''}

\paragraph{Response:} We \textbf{did not} make the argument in the paper, precisely because of the nuances (e.g., polynomial in what quantities; our analyses make assumptions that help bound quantities in \citet{uehara2022future}, so does that make \citet{uehara2022future}'s bound already polynomial? etc.), and instead described our results in technically concrete terms; but we stand by the sentiment of this claim. We made it in discussion only because some reviewer was asking for a table that summarizes existing results, which is common in well-investigated theoretical areas. 
We wanted to highlight  with a simple message (which, in hindsight, might not be the best move) that OPE in POMDPs is a new direction, and   few directly comparable results exist other than the work of \citet{uehara2022future} we build on.

%``Of course these claims are meaningless if we don't specify polynomial in what, but we have made that abundantly clear in the abstract, introduction, and our discussion here: by a polynomial bound we mean no exponential quantities such as the boundedness of cumulative importance weights''

\subsection*{Confounding}

\paragraph{Meta-review: } {\it ``when the behavior policy is history dependent, \ldots even when the reward function only depends on the current observation, there is still confounding issue because both the action and observed reward depends on the history.}

\paragraph{Response: } It is true that history is a confounder in a certain technical sense, \textbf{but this notion of confounding exists in almost every standard OPE setting, to the point it is meaningless to raise here}: even in a standard contextual bandit (CB) OPE problem \citep{li2010contextual}, context is a confounder in the sense that if we ignore context, the correlation between actions and rewards are spurious if behavior policy depends on the context. But these can be easily handled by accounting for the context in the estimator (e.g., fitting a reward model that depends on context, with a well-specified, i.e., realizable, reward class), and our case is not any different. 

What really distinguishes  between confounded and unconfounded POMDPs is \textbf{whether the behavior policy $\pib$ depends on privileged information not logged in the data}, such as the latent state. When all variables used by $\pib$ are observed in the data (which is clearly the case in our setting), sequential ignorability holds and there is no \textit{unobserved} confounding; see Section 3 of \citet{namkoong2020off}, Appendix B of \citet{uehara2022future}, and our  Appendix~\ref{app:related}. 

This discussion started with the reviewer raising a concern that we assume reward is a function of observation. They suspected that if reward is function of latent state, it would cause confounding issues.  We stand by our point during discussion: this is technically wrong, because we assume reward is observed, so all variables used by $\pib$ are still observed in the data. These observed variables block all the backdoor paths of the actions in the casual graph. Therefore, according to the backdoor criterion \citep{pearl2009causality}, the casual effect of the actions is identifiable and there is no unobserved confounding.
%
% because we assume the actions from the behavior policy only depend on the observations, thus observations blocks all the backdoor paths of the actions in the casual graph. According to the backdoor criterion \citep{pearl2009causality}, the casual effect of the actions is identifiable and there is no unobserved confounding issue. This is also stated in Appendix B in \citet{uehara2022future}. 
%
Furthermore, if reward depends on latent state (e.g., $r_h = R(s_h)$), we can always redefine the observation $o_h$ to be $(o_h, r_h)$ so that our assumption ($r_h$ is a function of $o_h$) is automatically satisfied, thus our current analyses already subsume this setting. 

\paragraph{Meta-review: } {\it ``To address the confounding issue, the authors only consider the class of memoryless policies, which bypasses the issue.''}

\paragraph{Response: } This is technically incorrect. \textbf{Our results, just as \citet{uehara2022future}, directly extend to history-dependent behavior and target policies}, which we mentioned both in the original manuscript and openreview discussion; see Appendix~\ref{app:fsm_policy} for more details. We focused on memoryless policies because this is the foundation for more general cases and already very challenging to analyze, with key theoretical concepts (such as belief and outcome coverage) missing in the literature. In the most general history-dependent case, the coverage parameters we identified may become exponential in the worst case, \textbf{but that has nothing to do with confounding.} 



\subsection*{Memoryless policies}
\paragraph{Meta-review: }  {\it ``this paper considers a rather restricted class of policies -- memoryless policies. Such a policy class seems never used in practice.''}

\paragraph{Response: } Again, we can handle fully general policies, just that in the worst case the coverage parameters may see exponential blow-up (Appendix~\ref{app:fsm_policy}). Also, memoryless (reactive) policies have always been the first thing researchers looked at in POMDP research; see the seminal works mentioned in Section 4.1 of \cite{murphy2000survey}.


\subsection*{MIS Algorithm and Experiments}
\paragraph{Meta-review: } {\it ``I think [the fact that the new algorithm only takes 1 page] is not a valid reason for not conducting numerical experiments \ldots  this algorithm is put as the second main contribution of this paper in the introduction. That seems to suggest that this new algorithm contributes to a half of the novelty. I would appreciate a more forthright response such as `the algorithm is only an information theoretical construction for understanding sample complexity', rather than massaging the importance assigned to each main result.''}

Our response was not intended to massage the importance of a main result only to get over the reviewer's concern, as we \textit{do} genuinely believe that the MIS algorithm is mostly a nice byproduct and cute observation. We have rewritten the introduction to better reflect the contributions of our work. That said, we also agree with the AC that ``the algorithm is only an information theoretical construction for understanding sample complexity'' is a nice way to put it, which does not conflict with our view of its importance. 


